Score Matching Riemannian Diffusion Means

Estimating means on Riemannian manifolds is generally computationally expensive because the Riemannian distance function is not known in closed-form for most manifolds. To overcome this, we show that Riemannian diffusion means can be efficiently estimated using score matching with the gradient of Brownian motion transition densities using the same principle as in Riemannian diffusion models. Empirically, we show that this is more efficient than Monte Carlo simulation while retaining accuracy and is also applicable to learned manifolds. Our method, furthermore, extends to computing the Fr\'echet mean and the logarithmic map for general Riemannian manifolds. We illustrate the applicability of the estimation of diffusion mean by efficiently extending Euclidean algorithms to general Riemannian manifolds with a Riemannian $k$-means algorithm and maximum likelihood Riemannian regression.

==> Sections/applications.tex <==
This section illustrates that using the Riemannian diffusion mean and given an extension of methods in Euclidean space to Riemannian manifolds these can now be computed efficiently to reduce time.

\paragraph{Error Analysis on the gradient} We can consider the gradient descent method as a discretized version of the following ODE system

\begin{equation*}
    \frac{\dif}{\dif t}\mu(t) = -v_{t}(\mu(t)), \quad \mu(0)=\mu_{0},
\end{equation*}

where $v_{t} = \nabla \log p_{t}(x)$. Let $\mu_{0}$ be random, then it follows that $\mu(t)$ will have the same distribution as $p_{t}$ if $\mu_{0}$ has the density of $p_{0}$, which denote the probability density of Brownian motion [REFERENCE HERE]. Correspondingly we can define $\frac{\dif}{\dif t}\tilde{\mu}'(t) = -\tilde{v}_{t}(\tilde{\mu}(t)), \quad \tilde{\mu}(0)=\mu_{0}$ with $\tilde{v}_{t}=s_{\theta}$ as the corresponding ODE using the score.

By [REFERENCE] we have that with initial distribution $\pi$

\begin{equation*}
    \mathrm{kl}(p|\mu(T)) - \mathrm{kl}(p_{T}|\pi)) \leq \int_{0}^{T}\mathbb{E}\left[|\nabla \log p_{t}(X_{t}) - \nabla \log q_{t}(X_{t})|^{2}+|\nabla \log q_{t}(X_{t})-s(t,X_{t})|^{2}\right]\,\dif t
\end{equation*}

Clearly if the score is equal to $\nabla \log p$ the above bound will be zero. \citet{eltzner2022diffusion} shows that the estimator of the diffusion t-mean will converge in distribution to a normal distribution with convergence rate of $\sqrt{n}$.


As a first simple (Euclidean) example assume that $|s_{\theta}-\nabla \log p| < \epsilon$ for all $t,x$. Let $\tilde{\mu}_{i}$ denote the $i$th update step with gradient descent using $s_{\theta}$, and let $\mu_{i}$ denote the $i$th update step with $\nabla \log p$. Assume that both gradient methods start with $\mu_{0}=\tilde{mu}_{0}=x_{0}$, then

\begin{equation*}
    \begin{split}
        |\tilde{\mu}_{i+1}-\mu_{i+1}| &= |\tilde{\mu}_{i+1}-\mu_{i+1}| \\
        &= |\tilde{\mu}_{i}-\frac{\tau}{N}\sum_{i=1}^{N}s_{\theta}(x_{i})-\mu_{i}+\frac{\tau}{N}\sum_{i=1}^{N}\nabla \log p(x_{i})| \\
        &\leq |\tilde{\mu}_{i}-\mu_{i}| + \frac{\tau}{N}\sum_{i=1}^{N}|\nabla \log p(x_{i}) - s_{\theta}(x_{i})| \\
        &= |\tilde{\mu}_{i}-\mu_{i}| + \tau \epsilon \\
        &\leq ... \\
        &\leq |\tilde{\mu}_{0}-\mu_{0}| + i\tau \epsilon \\
        &= i\tau \epsilon.
    \end{split}
\end{equation*}

So clearly, in the Euclidean case we see that if $\epsilon \rightarrow 0$, then the diffusion mean will converge to the true diffusion mean by gradient descent. Further, if the algorithm converges "fast" in the sense that $n_{\mathrm{iter}}$ is low, then $|\tilde{\mu}_{i+1}-\mu_{i+1}|$ will be close assuming that the step size $\tau$ and $\epsilon$ is close. However, if the algorithm is slow to converge, then the uncertainty will increase. Similarly we can for gradient descent of Riemannian manifolds observe that

\begin{equation*}
    \begin{split}
        \dist^{2}\left(\tilde{\mu}_{i+1}, \mu_{i+1}\right) &= \dist^{2}\left(\mathrm{Exp}_{\tilde{\mu_{i}}}\left(-\tau s_{\theta}\right), \mathrm{Exp}_{\mu_{i}}\left(-\tau \nabla \log p\right)\right) \\
        &= \mathrm{SOMETHING HERE}
    \end{split}
\end{equation*}

Some ideas

\begin{equation*}
    \dist^{2}\left(\mathrm{Exp}_{\mu_{0}}\left(-\tau s_{\theta}\right), \mathrm{Exp}_{\mu_{0}}\left(-\tau \nabla \log p\right)\right) = \tau^{2}\norm{\nabla \log p-s_{\theta}}^{2}-\frac{1}{3}R(\nabla \log p, s_{\theta}, s_{\theta}, \nabla \log p)\tau^{4}+O(\tau^{5})
\end{equation*}

\paragraph{Estimating Fréchet Mean} The Fréchet mean is given by $\mu^{\text{Fréchet}}(x_{1:N}) = \argmin_{\mu \in \mathcal{M}} \mathbb{E}\left[\dist^{2}(X,\mu)\right]$ \citep{frechet1948} with $\nabla_{\mu}\mathbb{E}\left[\dist^{2}(X,\mu)\right] = \mathbb{E}\left[2\text{Log}_{\mu}(X)\right]$ \citep{pennec2006statriemann}. By \citet{hsustochastic} it follows that $\lim_{t \downarrow 0} t \log p(x,y,t) = -\frac{\dist^{2}\left(x,y\right)}{2}$ uniformly. Since the convergence is uniform, then (I think uniform convergence is enough for this to hold)

\begin{equation}
    -\lim_{t \downarrow 0} t \nabla_{y}\log p(x,y,t) = \text{Log}_{y}(x).
    \label{eq:learned_log}
\end{equation}

Thus given the learned gradient and choosing a sufficiently small $t>0$, the Fréchet mean can similarly be estimated using gradient-descent approaches. Note that given the log gradient only has to be estimated for a single value of $t$, then it is possible to train the score matching neural network only for this value of $t$ to increase accuracy in training.

\paragraph{Estimating the Heat Kernel} 
The heat equation, $\frac{d}{dt}p(x,y,t)=\frac{1}{2}\nabla_{x}p(x,y,t)$, can be re-written as a transport equation \citep{boffi2023probability}

\begin{equation*}
    2
\end{equation*}

\paragraph{Estimating the Heat Kernel}
The heat kernel can equivalently be written as \citep{hsustochastic} $p(x,y,t) = \left(\frac{1}{2\pi t}\right)^{d/2}e^{-\frac{\dist^{2}(x,y)}{2t}}\sum_{n=0}^{\infty}H_{n}(x,y)t^{n}$. Thus,

\begin{equation*}
    \log p(x,y,t) = \log\sum_{n=0}^{\infty}H_{n}(x,y)t^{n}-\frac{\dist^{2}(x,y)}{2t}-\frac{d}{2}\log\left(2\pi t\right),
\end{equation*}

which implies that

\begin{equation*}
    \begin{split}
        \nabla_{y} \log p(x,y,t) &= \nabla_{y} \left(\log\sum_{n=0}^{\infty}H_{n}(x,y)t^{n}-\frac{\dist^{2}(x,y)}{2t}-\frac{d}{2}\log\left(2\pi t\right)\right) \\
        &= \frac{\nabla_{y}\sum_{n=0}^{\infty}H_{n}(x,y)t^{n}}{\sum_{n=0}^{\infty}H_{n}(x,y)t^{n}}-\frac{2\text{Log}_{y}(x)}{2t} \\
        &\Leftrightarrow \nabla_{y}\sum_{n=0}^{\infty}H_{n}(x,y)t^{n} = \sum_{n=0}^{\infty}H_{n}(x,y)t^{n}\left(\nabla_{y} \log p(x,y,t)+\frac{2\text{Log}_{y}(x)}{2t}\right)
    \end{split}
\end{equation*}

The above is equivalent to the differential equation

\begin{equation*}
    \nabla_{y}f(x,y,t) = f(x,y,t)g(x,y,t),
\end{equation*}

where $f(x,y,t):=\sum_{n=0}^{\infty}H_{n}(x,y)t^{n}$ and $g(x,y,t):=\nabla_{y} \log p(x,y,t)+\frac{2\text{Log}_{y}(x)}{2t}$. Thus for each fixed $x \in \mathcal{M},t \in \mathbb{R}$ the heat kernel can be estimated for each $y$ by solving the above differential equation in one variable. Assume "panserformlen" holds in the multidimensional case, then the solution is 

\begin{equation*}
    \nabla_{y}\sum_{n=0}^{\infty}H_{n}(x,y)t^{n} = c\exp\left(-\int \left(\nabla_{y} \log p(x,y,t)+\frac{2\text{Log}_{y}(x)}{2t}\right) \,dy \right)
\end{equation*}

\paragraph{Riemannian K-means} The Euclidean $k$-means algorithm is an unsupervised learning \citep{bishop}, which has been generalized into a Riemmannian setting \citep{arvanitidis2018latent}. The objective is to choose $K$-clusters, $\{\mu_{k}\}_{k=1}^{K}$, and assign each data point to exactly one cluster, i.e.

\begin{equation*}
    \begin{split}
        \min_{\mu \in \mathcal{M}, z \in \{0,1\}} \quad &\sum_{i=1}^{N}\sum_{k=1}^{K} z_{ik} \dist^{2}\left(x_{i},\mu_{k}\right) \\
        \text{s.t.} \quad &\sum_{k=1}^{K}z_{ik}=1, \quad \forall i \in \{1,\dots,N\}.
    \end{split}
\end{equation*}

Equivalently to the Euclidean case the clusters can be updated as the Fréchet mean estimated using gradient-descent as in algorithm \ref{al:est_diffusion_mean}, but using the gradient in eq. \ref{eq:learned_log}.

\paragraph{Riemannian K-means}. The Euclidean $k$-means algorithm is an unsupervised learning \citep{bishop}, which has been generalized into a Riemmannian setting \citep{arvanitidis2018latent}. It consists of initializing K centroids and then assign each data point to the cluster of the closest centroid, and then iteratively updating the centroid of each cluster as the mean value of data points in the cluster to minimize $\sum_{i=1}^{N}\sum_{k=1}^{K} \delta_{ik}||x_{i}-\mu_{k}||^{2}$ with $\{x_{i}\}_{i=1}^{N}$ denoting the observations. Rather than minimizing the squared distances we propose to minimize the transition densities of a Wiener process, $\sum_{i=1}^{N}\sum_{k=1}^{K} \delta_{ik} \ln p(x_{i}, \mu_{k}, t)$. This is minimized heuristically using the following approach: the centroids are updated using the diffusion mean and rather than estimating the distance between each data point and each centroid this is estimated as the smallest time $t = \argmin_{t_{0}>0} ||\frac{\dif}{\dif t}\ln p\left(x_{i},\mu_{j},t\right)||$, which can be estimated by eq. \ref{eq:time_derivative}. The observations, $x_{i}$, are then assigned to the centroid with the smallest diffusion time. The algorithm is written in algortihm \ref{al:rm_kmeans}.

\begin{algorithm}
    \SetAlgoLined
    \textbf{Input}: K, $N_{\text{iter}}$, $t$, $\{\mu_{i}^{\text{init}}\}_{i=1}^{K}$, $\{x_{i}\}_{i=1}^{N_{\text{data}}}$ \\
    \textbf{Output}: $\mu_{t}^{\text{Diffusion}}$ \\
    Learn neural network $s_{\theta}$ minimizing eq. \ref{eq:score_loss_fun} \\
    Set $\{\mu_{i}^{(0)}\}_{i=1}^{K} = \{\mu_{(i)}^{\text{init}}\}_{i=1}^{K}$ \\
    \For{i=1,\dots,$N_{\text{iter}}$} {
        \For{j=1,\dots,$K$} {
            \For{l=1,\dots,$N_{\text{data}}$} {
                Set $t_{l} = \argmin_{t>0} ||\frac{\dif}{\dif t}\ln p\left(x_{i},\mu_{j}^{(i)},t\right)||$ using eq. \ref{eq:time_derivative} for the approximation $s_{\theta}$ \\
            }
            Assign $x_{j}$ to cluster $k=\argmin_{l} t_{l}$ \\
        }
        Set $\mu_{k}^{(i})$ as the diffusion mean using algortihm \ref{al:est_diffusion_mean} for all $\{x_{j}\}_{j=1}^{N_{\text{data}}}$ in cluster $k$.
    }
    return $\{\mu_{i}^{N_{\text{iter}}}\}_{i=1}^{K}$ \\
    \caption{Riemannian $k$-Diffusion Means}
    \label{al:rm_kmeans}
\end{algorithm}

To reduce the complexity of the algorithm the diffusion mean is estimated using only a steepest descent method.

\paragraph{Riemannian Principal Curves} is a generalization of Euclidean principal curves \citep{hastie_pc} to a Riemannian setting \citep{haubergprincurves}. Riemannian principal curves informally estimate a smooth curve that runs through the center of the observed data. Following \citet{haubergprincurves} let $c: \mathbb{R}_{+} \rightarrow \mathcal{M}$ be a curve that has been discretized to a set of points, $c_{1:T}=(c(1),\dots,c(T))$ for some $T \in \mathbb{N}$ and let $k$ denote a smooth kernel, then the principal curves are iteratively updated as:

\begin{equation*}
    c^{(i)}(t) = \argmin_{x} \sum_{n=1}^{N} w_{t,n}\dist^{2}(x_{n},x), \quad w_{t,n} = k\left(\frac{\dist(c^{i-1}(t),c^{i-1}(\hat{t}_{n}))}{\sigma}\right),
\end{equation*}

where $\hat{t}_{n} = \argmin_{t \in \{1,\dots,T\}} \dist(c(t),x_{n})$ for all $n$. Rather than estimating the curve $c$ using the Fréchet mean this can equivalently be done in the context of the diffusion mean, which gives rise to the following algorithm:

\begin{equation}
    c^{(i)}(t) = \argmin_{x} \sum_{n=1}^{N} -w_{t,n}\ln p(x, x_{n}, \tilde{t}), \quad w_{t,n} = k\left(\frac{||\frac{d}{dt}s_{\theta}c^{i-1}(t),c^
 {i-1}(t_{n}), t^{\text{diffusion}}||}{\sigma}\right)
 \label{eq:rm_pcurve}
\end{equation}

with $\hat{t}_{n} = \argmin_{t \in \{1,\dots,T\}} ||\frac{\dif}{\dif t}s_{\theta}(c(t),x_{n},t^{\text{diffusion}}||$. Thus we approximate points close to each other as those points, where the gradient of the diffusion time is relatively low. In this context the diffusion time is set as a hyper-parameter.

\paragraph{Estimating the Cut Locus} Follow-up on the behavior of exploding gradients on the cut locus, see \citet{neel2004} and \citet{neel2006small} to see if its possible to estimate the cut locus given the learned gradients.

\paragraph{Variance Reducing Gradient Descent} Assume that we have estimated a neural network, $s_{\theta}(x,y,t)$ such that

\begin{equation*}
    s_{\theta}(x,y,t) = \nabla \ln p(x,y,t) + \epsilon_{x,y,t},
\end{equation*}

where $\epsilon_{x,y,t}$ are a i.i.d. realized random variables with $\mathbb{E}\left[\epsilon_{x,y,t}\right] = 0$. Assume the update step

\begin{equation*}
    \mu^{(k+1)} = mu^{(k)}+s_{\theta}(x,y,t)) = \mu^{(k)}+\nabla \ln p(x,y,t))+\epsilon_{x,y,t},
\end{equation*}

then by the central limit theorem it follows that the sequence

\begin{equation*}
    \bar{\mu}^{(k+1)} = \frac{1}{N}\sum_{i=j}^{N} \left(\mu^{(k)}+s_{\theta}(x,y,t))\right)
\end{equation*}

will converge to the optimum without noise for sufficiently high $N$, where $\{\mu_{j}\}$ denotes $N$ different point on the manifold. Thus by starting the gradient descent an averaging over them, the algorithm will converge. This will work in Euclidean space, while for Manifolds the approach has to be performed in the tangent spaces. The method is also numerically expensive, since it requires estimating $N$ gradients at each iteration. Note that if the gradient descent method is close to optimum for one gradient such that it is only white noise that differs between the true optimum and the gradient descent approach, then the average of $N$ further gradient descent step can be taken.

Alternative ideas could be to use to have multiple networks and then take the mean of each network. Alternatively if possible try to learn the distribution (maybe through Bayesian networks).

\paragraph{Further Applications} The following contains a list of further directly applicable models on Riemannian manifolds that can be extended using the Riemannian scores

\begin{itemize}
    \item Geodesic regression \citep{fletcher:geodesicregression:2013} uses distances and the Logaritmic map, both of which can be estimated using the above methods. Further the geodesic regression can re-written using the Riemannian Brownian Motion for a probabilistic version.
    \item Riemannian Principal Curves \citep{haubergprincurves} also uses distance based loss-function, which can either be approximated by the above methods or re-formualated as using the log density of the Riemannian Brownian Motion.
    \item Wrapped Gaussian Processes \citep{feragenwgp} makes of the Logaritmic map to compute the Wrapped Gaussian Process, which can be approximated using the above methods. Similarly this could mostly be extended using a Wrapped Brownian Motion approach or directly using a Riemannian Brownian Bridge through the data.
\end{itemize}
